Pareto Curves for Probabilistic Model Checking

Multi-objective probabilistic model checking provides a way to verify several, possibly conflicting, quantitative properties of a stochastic system. It has useful applications in controller synthesis and compositional probabilistic verification. However, existing methods are based on linear programming, which limits the scale of systems that can be analysed and makes verification of time-bounded properties very difficult. We present a novel approach that addresses both of these shortcomings, based on the generation of successive approximations of the Pareto curve for a multi-objective model checking problem. We illustrate dramatic improvements in efficiency on a large set of benchmarks and show how the ability to visualise Pareto curves significantly enhances the quality of results obtained from current probabilistic verification tools.

==> concl.tex <==
\vspace*{-0.4cm}
\section{Conclusions}\label{concl-sect}

\vspace*{-0.2cm}
We have presented novel techniques for multi-objective model checking of MDPs,
using a value iteration-based computation to build successive approximations of the Pareto curve.
%based on generation of successive approximations of the Pareto curve using value iteration.
Compared to existing approaches, this gives significant gains in efficiency and scalability,
and enables verification of time-bounded properties.
Furthermore, we showed the benefits of visualising the Pareto curve
for several probabilistic model checking case studies.
%
Future directions include extending our techniques
to timed probabilistic models such as CTMDPs and PTAs.


==> figures/graph3d.tex <==
\begin{tikzpicture}[scale=0.3,x = {(-4.499513cm,-1.834018cm)}, y = {(0cm,6.577848cm)},z = {(2.304853cm,-0.661467cm)},font=\scriptsize]
\tikzstyle{every node}+=[font=\tiny]
\draw[-latex'] (0,0,0) -- (0,0,2.4465306122448984);
\draw[-latex'] (0,0,0) -- (0,1.1200000000000006,0);
\draw[-latex'] (0,0,0) -- (1.1200000000000006,0,0);
\draw (0.5,0,0) -- (0.5,0.04,0) node[above, inner sep=1pt] {0.5};
\draw (1.0,0,0) -- (1.0,0.04,0) node[above, inner sep=1pt] {1};
\draw (0,0.5,0) -- (0.04,0.5,0) node[left, inner sep=1pt] {0.5};
\draw (0,1.0,0) -- (0.04,1.0,0) node[left, inner sep=1pt] {1};
\draw (0,0,0.5) -- (0,0.04,0.5) node[above, inner sep=1pt] {0.5};
\draw (0,0,1.0) -- (0,0.04,1.0) node[above, inner sep=1pt] {1};
\draw (0,0,1.5) -- (0,0.04,1.5) node[above, inner sep=1pt] {1.5};
\draw (0,0,2.0) -- (0,0.04,2.0) node[above, inner sep=1pt] {2};
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.7551020408163269, 0.0, 2.326530612244897) -- (0.0, 0.7551020408163269, 2.3265306122448965) -- (0.0, 0.0, 2.3265306122448983) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.2448979591836734, 0.9999999999999997, 0.0) -- (0.0, 1.0000000000000007, 0.0) -- (0.0, 1.0000000000000007, 2.020408163265302) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.0, 0.0) -- (1.0000000000000007, 0.24489795918366936, 0.0) -- (1.0000000000000007, 0.0, 2.0204081632653015) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.7551020408163269, 0.0, 2.326530612244897) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.0, 0.7551020408163269, 2.3265306122448965) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.9387755102040825, 0.0, 2.142857142857143) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.7551020408163269, 0.0, 2.326530612244897) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.8775510204081638, 0.3673469387755106, 0.0) -- (0.2448979591836734, 0.9999999999999997, 0.0) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.24489795918366936, 0.0) -- (0.8775510204081638, 0.3673469387755106, 0.0) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.0, 1.0000000000000007, 2.020408163265302) -- (0.0, 0.9387755102040825, 2.142857142857141) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.2448979591836734, 0.9999999999999997, 0.0) -- (0.0, 1.0000000000000007, 2.020408163265302) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.2448979591836734, 0.9999999999999997, 0.0) -- (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.0, 2.0204081632653015) -- (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- (0.9387755102040825, 0.0, 2.142857142857143) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.24489795918366936, 0.0) -- (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- (1.0000000000000007, 0.0, 2.0204081632653015) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.24489795918366936, 0.0) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- cycle;
%\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- cycle;
%\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- cycle;
%\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- cycle;
%\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- cycle;
%\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.9387755102040825, 0.0, 2.142857142857143) -- (0.7551020408163269, 0.2448979591836734, 2.326530612244897) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- cycle;
%\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.7551020408163269, 0.2448979591836734, 2.326530612244897) -- (0.9387755102040825, 0.0, 2.142857142857143) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.48979591836734715, 0.7551020408163269, 2.3265306122448965) -- (0.0, 0.9387755102040825, 2.142857142857141) -- (0.0, 0.7551020408163269, 2.3265306122448965) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.48979591836734715, 0.7551020408163269, 2.3265306122448965) -- (0.0, 0.7551020408163269, 2.3265306122448965) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.48979591836734715, 0.7551020408163269, 2.3265306122448965) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.9387755102040825, 0.30612244897959184, 2.1428571428571392) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.9387755102040825, 0.0, 2.142857142857143) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- (0.9387755102040825, 0.30612244897959184, 2.1428571428571392) -- (0.9387755102040825, 0.0, 2.142857142857143) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.9387755102040825, 0.30612244897959184, 2.1428571428571392) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.2448979591836734, 0.9387755102040825, 2.142857142857141) -- (0.0, 0.9387755102040825, 2.142857142857141) -- (0.48979591836734715, 0.7551020408163269, 2.3265306122448965) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.0, 0.9387755102040825, 2.142857142857141) -- (0.2448979591836734, 0.9387755102040825, 2.142857142857141) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.30612244897959184, 0.9387755102040825, 2.1428571428571406) -- (0.2448979591836734, 0.9387755102040825, 2.142857142857141) -- (0.48979591836734715, 0.7551020408163269, 2.3265306122448965) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.30612244897959184, 0.9387755102040825, 2.1428571428571406) -- (0.48979591836734715, 0.7551020408163269, 2.3265306122448965) -- cycle;
\path[fill, line width=0pt, opacity=0.3, color=gray!40] (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.2448979591836734, 0.9387755102040825, 2.142857142857141) -- (0.30612244897959184, 0.9387755102040825, 2.1428571428571406) -- cycle;
\draw[color=gray] (0.7551020408163269, 0.0, 2.326530612244897) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934);
\draw[color=gray] (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.0, 1.0000000000000007, 2.020408163265302);
\draw[color=gray] (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.2448979591836734, 0.9999999999999997, 0.0);
\draw[color=gray] (1.0000000000000007, 0.0, 2.0204081632653015) -- (1.0000000000000007, 0.2448979591836734, 2.0204081632653077);
\draw[color=gray] (1.0000000000000007, 0.24489795918366936, 0.0) -- (1.0000000000000007, 0.2448979591836734, 2.0204081632653077);
\draw[color=gray] (0.48979591836734715, 0.7551020408163269, 2.3265306122448965) -- (0.0, 0.7551020408163269, 2.3265306122448965);
\draw[color=gray] (0.7551020408163269, 0.48979591836734715, 2.3265306122448934) -- (0.48979591836734715, 0.7551020408163269, 2.3265306122448965);
\draw[color=gray] (0.9387755102040825, 0.30612244897959184, 2.1428571428571392) -- (0.9387755102040825, 0.0, 2.142857142857143);
\draw[color=gray] (0.9387755102040825, 0.30612244897959184, 2.1428571428571392) -- (0.7551020408163269, 0.48979591836734715, 2.3265306122448934);
\draw[color=gray] (1.0000000000000007, 0.2448979591836734, 2.0204081632653077) -- (0.9387755102040825, 0.30612244897959184, 2.1428571428571392);
\draw[color=gray] (0.2448979591836734, 0.9387755102040825, 2.142857142857141) -- (0.0, 0.9387755102040825, 2.142857142857141);
\draw[color=gray] (0.30612244897959184, 0.9387755102040825, 2.1428571428571406) -- (0.48979591836734715, 0.7551020408163269, 2.3265306122448965);
\draw[color=gray] (0.30612244897959184, 0.9387755102040825, 2.1428571428571406) -- (0.2448979591836734, 0.9387755102040825, 2.142857142857141);
\draw[color=gray] (0.2448979591836734, 0.9999999999999998, 2.0204081632653073) -- (0.30612244897959184, 0.9387755102040825, 2.1428571428571406);

\path[-latex'] (0,0,0) -- (0,0,2.4465306122448984) node[pos=1, above] {$z$};
\path[-latex'] (0,0,0) -- (0,1.1200000000000006,0) node[pos=0.95, right] {$y$};;
\path[-latex'] (0,0,0) -- (1.1200000000000006,0,0) node[pos=0.9, below] {$x$};;
\end{tikzpicture}

